Probing Source and Detector NSI parameters at the DUNE Near Detector

We investigate the capability of the DUNE Near Detector (ND) to constrain Non Standard Interaction parameters (NSI) describing the production of neutrinos ($\varepsilon_{\alpha\beta}^s$) and their detection ($\varepsilon_{\alpha\beta}^d$). We show that the DUNE ND is able to reject a large portion of the parameter space allowed by DUNE Far Detector analyses and to set the most stringent bounds from accelerator neutrino experiments on $|\varepsilon_{\mu e}^{s,d}|$ for wide intervals of the related phases. We also provide simple analytic understanding of our results as well as a numerical study of their dependence on the systematic errors, showing that the DUNE ND offers a clean environment where to study source and detector NSI.

==> bib.tex <==
\begin{thebibliography}{00}

%\cite{Abe:2019vii}
\bibitem{Abe:2019vii}
K.~Abe \textit{et al.} [T2K],
%``Constraint on the matter–antimatter symmetry-violating phase in neutrino oscillations,''
Nature \textbf{580} (2020) no.7803, 339-344
doi:10.1038/s41586-020-2177-0
[arXiv:1910.03887 [hep-ex]].
%26 citations counted in INSPIRE as of 12 May 2020

%\cite{Esteban:2018azc}
\bibitem{Esteban:2018azc}
I.~Esteban, M.~Gonzalez-Garcia, A.~Hernandez-Cabezudo, M.~Maltoni and T.~Schwetz,
%``Global analysis of three-flavour neutrino oscillations: synergies and tensions in the determination of $\theta_{23}$, $\delta_{CP}$, and the mass ordering,''
JHEP \textbf{01} (2019), 106
doi:10.1007/JHEP01(2019)106
[arXiv:1811.05487 [hep-ph]].
%364 citations counted in INSPIRE as of 12 May 2020

%\cite{deSalas:2017kay}
\bibitem{deSalas:2017kay}
P.~de Salas, D.~Forero, C.~Ternes, M.~Tortola and J.~Valle,
%``Status of neutrino oscillations 2018: 3$\sigma$ hint for normal mass ordering and improved CP sensitivity,''
Phys. Lett. B \textbf{782} (2018), 633-640
doi:10.1016/j.physletb.2018.06.019
[arXiv:1708.01186 [hep-ph]].
%464 citations counted in INSPIRE as of 12 May 2020

  %\cite{Grossman:1995wx}
\bibitem{Grossman:1995wx} 
  Y.~Grossman,
  %``Nonstandard neutrino interactions and neutrino oscillation experiments,''
  Phys.\ Lett.\ B {\bf 359}, 141 (1995)
  doi:10.1016/0370-2693(95)01069-3
  [hep-ph/9507344].
  %%CITATION = doi:10.1016/0370-2693(95)01069-3;%%
  %174 citations counted in INSPIRE as of 19 Mar 2020

%\cite{Roulet:1991sm}
\bibitem{Roulet:1991sm} 
  E.~Roulet,
  %``MSW effect with flavor changing neutrino interactions,''
  Phys.\ Rev.\ D {\bf 44}, R935 (1991).
  doi:10.1103/PhysRevD.44.R935
  %%CITATION = doi:10.1103/PhysRevD.44.R935;%%
  %242 citations counted in INSPIRE as of 19 Mar 2020
  
  %\cite{Guzzo:1991hi}
\bibitem{Guzzo:1991hi} 
  M.~M.~Guzzo, A.~Masiero and S.~T.~Petcov,
  %``On the MSW effect with massless neutrinos and no mixing in the vacuum,''
  Phys.\ Lett.\ B {\bf 260}, 154 (1991).
  doi:10.1016/0370-2693(91)90984-X
  %%CITATION = doi:10.1016/0370-2693(91)90984-X;%%
  %301 citations counted in INSPIRE as of 19 Mar 2020
  
  %\cite{Bergmann:1999rz}
\bibitem{Bergmann:1999rz} 
  S.~Bergmann, Y.~Grossman and E.~Nardi,
  %``Neutrino propagation in matter with general interactions,''
  Phys.\ Rev.\ D {\bf 60}, 093008 (1999)
  doi:10.1103/PhysRevD.60.093008
  [hep-ph/9903517].
  %%CITATION = doi:10.1103/PhysRevD.60.093008;%%
  %77 citations counted in INSPIRE as of 19 Mar 2020
  

    %\cite{Kopp:2007ne}
\bibitem{Kopp:2007ne} 
  J.~Kopp, M.~Lindner, T.~Ota and J.~Sato,
  %``Non-standard neutrino interactions in reactor and superbeam experiments,''
  Phys.\ Rev.\ D {\bf 77}, 013007 (2008)
  doi:10.1103/PhysRevD.77.013007
  [arXiv:0708.0152 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.77.013007;%%
  %188 citations counted in INSPIRE as of 19 Mar 2020  
  
  %\cite{Coloma:2017ncl}
\bibitem{Coloma:2017ncl}
P.~Coloma, M.~Gonzalez-Garcia, M.~Maltoni and T.~Schwetz,
%``COHERENT Enlightenment of the Neutrino Dark Side,''
Phys. Rev. D \textbf{96} (2017) no.11, 115007
doi:10.1103/PhysRevD.96.115007
[arXiv:1708.02899 [hep-ph]].
%63 citations counted in INSPIRE as of 21 Apr 2020

%\cite{Khan:2017oxw}
\bibitem{Khan:2017oxw}
A.~N.~Khan and D.~W.~McKay,
%``$\sin^2(\theta)w$ estimate and bounds on nonstandard interactions at source and detector in the solar neutrino low-energy regime,''
JHEP \textbf{07}, 143 (2017)
doi:10.1007/JHEP07(2017)143
[arXiv:1704.06222 [hep-ph]].
%10 citations counted in INSPIRE as of 05 Jun 2020

%\cite{Liao:2017uzy}
\bibitem{Liao:2017uzy}
J.~Liao and D.~Marfatia,
%``COHERENT constraints on nonstandard neutrino interactions,''
Phys. Lett. B \textbf{775} (2017), 54-57
doi:10.1016/j.physletb.2017.10.046
[arXiv:1708.04255 [hep-ph]].
%58 citations counted in INSPIRE as of 21 Apr 2020
  
  
%\cite{Bolanos:2008km}
\bibitem{Bolanos:2008km}
A.~Bolanos, O.~Miranda, A.~Palazzo, M.~Tortola and J.~Valle,
%``Probing non-standard neutrino-electron interactions with solar and reactor neutrinos,''
Phys. Rev. D \textbf{79} (2009), 113012
doi:10.1103/PhysRevD.79.113012
[arXiv:0812.4417 [hep-ph]].
%83 citations counted in INSPIRE as of 21 Apr 2020   
  
%\cite{Agarwalla:2012wf}
\bibitem{Agarwalla:2012wf}
S.~K.~Agarwalla, F.~Lombardi and T.~Takeuchi,
%``Constraining Non-Standard Interactions of the Neutrino with Borexino,''
JHEP \textbf{12} (2012), 079
doi:10.1007/JHEP12(2012)079
[arXiv:1207.3492 [hep-ph]].
%21 citations counted in INSPIRE as of 21 Apr 2020



%\cite{GonzalezGarcia:2011my}
\bibitem{GonzalezGarcia:2011my}
M.~Gonzalez-Garcia, M.~Maltoni and J.~Salvado,
%``Testing matter effects in propagation of atmospheric and long-baseline neutrinos,''
JHEP \textbf{05} (2011), 075
doi:10.1007/JHEP05(2011)075
[arXiv:1103.4365 [hep-ph]].
%71 citations counted in INSPIRE as of 21 Apr 2020

%\cite{Salvado:2016uqu}
\bibitem{Salvado:2016uqu}
J.~Salvado, O.~Mena, S.~Palomares-Ruiz and N.~Rius,
%``Non-standard interactions with high-energy atmospheric neutrinos at IceCube,''
JHEP \textbf{01} (2017), 141
doi:10.1007/JHEP01(2017)141
[arXiv:1609.03450 [hep-ph]].
%30 citations counted in INSPIRE as of 21 Apr 2020


  %\cite{Biggio:2009nt}
\bibitem{Biggio:2009nt} 
  C.~Biggio, M.~Blennow and E.~Fernandez-Martinez,
  %``General bounds on non-standard neutrino interactions,''
  JHEP {\bf 0908}, 090 (2009)
  doi:10.1088/1126-6708/2009/08/090
  [arXiv:0907.0097 [hep-ph]].
  %%CITATION = doi:10.1088/1126-6708/2009/08/090;%%
  %223 citations counted in INSPIRE as of 19 Mar 2020
  
  %\cite{Agarwalla:2014bsa}
\bibitem{Agarwalla:2014bsa}
S.~K.~Agarwalla, P.~Bagchi, D.~V.~Forero and M.~Tórtola,
%``Probing Non-Standard Interactions at Daya Bay,''
JHEP \textbf{07} (2015), 060
doi:10.1007/JHEP07(2015)060
[arXiv:1412.1064 [hep-ph]].
%24 citations counted in INSPIRE as of 21 Apr 2020  


%\cite{Adamson:2013ovz}
\bibitem{Adamson:2013ovz}
P.~Adamson \textit{et al.} [MINOS],
%``Search for flavor-changing non-standard neutrino interactions by MINOS,''
Phys. Rev. D \textbf{88} (2013) no.7, 072011
doi:10.1103/PhysRevD.88.072011
[arXiv:1303.5314 [hep-ex]].
%47 citations counted in INSPIRE as of 21 Apr 2020 

%\cite{Ohlsson:2012kf}
\bibitem{Ohlsson:2012kf} 
  T.~Ohlsson,
  %``Status of non-standard neutrino interactions,''
  Rept.\ Prog.\ Phys.\  {\bf 76}, 044201 (2013)
  doi:10.1088/0034-4885/76/4/044201
  [arXiv:1209.2710 [hep-ph]].
  %%CITATION = doi:10.1088/0034-4885/76/4/044201;%%
  %220 citations counted in INSPIRE as of 19 Mar 2020
  
  %\cite{Dev:2019anc}
\bibitem{Dev:2019anc} 
  P.~S.~Bhupal Dev {\it et al.},
  %``Neutrino Non-Standard Interactions: A Status Report,''
  SciPost Phys.\ Proc.\  {\bf 2}, 001 (2019)
  doi:10.21468/SciPostPhysProc.2.001
  [arXiv:1907.00991 [hep-ph]].
  %%CITATION = doi:10.21468/SciPostPhysProc.2.001;%%
  %25 citations counted in INSPIRE as of 19 Mar 2020
  
    
%\cite{Giunti:2019xpr}
\bibitem{Giunti:2019xpr}
C.~Giunti,
%``General COHERENT constraints on neutrino nonstandard interactions,''
Phys. Rev. D \textbf{101} (2020) no.3, 035039
doi:10.1103/PhysRevD.101.035039
[arXiv:1909.00466 [hep-ph]].
%11 citations counted in INSPIRE as of 21 Apr 2020

%\cite{Khan:2016uon}
\bibitem{Khan:2016uon}
A.~N.~Khan,
%``Global analysis of the source and detector nonstandard interactions using the short baseline ν-e and ν¯-e scattering data,''
Phys. Rev. D \textbf{93}, no.9, 093019 (2016)
doi:10.1103/PhysRevD.93.093019
[arXiv:1605.09284 [hep-ph]].
%25 citations counted in INSPIRE as of 05 Jun 2020

%\cite{Coloma:2019mbs}
\bibitem{Coloma:2019mbs}
P.~Coloma, I.~Esteban, M.~Gonzalez-Garcia and M.~Maltoni,
%``Improved global fit to Non-Standard neutrino Interactions using COHERENT energy and timing data,''
JHEP \textbf{02} (2020), 023
doi:10.1007/JHEP02(2020)023
[arXiv:1911.09109 [hep-ph]].
%12 citations counted in INSPIRE as of 21 Apr 2020


%\cite{Dutta:2020che}
\bibitem{Dutta:2020che} 
  B.~Dutta, R.~F.~Lang, S.~Liao, S.~Sinha, L.~Strigari and A.~Thompson,
  %``A global analysis strategy to resolve neutrino NSI degeneracies with scattering and oscillation data,''
  arXiv:2002.03066 [hep-ph].
  %%CITATION = ARXIV:2002.03066;%%
  %2 citations counted in INSPIRE as of 19 Mar 2020
  
  % -------------NSI long baseline----------


%\cite{Adhikari:2012vc}
\bibitem{Adhikari:2012vc}
R.~Adhikari, S.~Chakraborty, A.~Dasgupta and S.~Roy,
%``Non-standard interaction in neutrino oscillations and recent Daya Bay, T2K experiments,''
Phys. Rev. D \textbf{86} (2012), 073010
doi:10.1103/PhysRevD.86.073010
[arXiv:1201.3047 [hep-ph]].
%25 citations counted in INSPIRE as of 21 Apr 2020

%\cite{Coelho:2012bp}
\bibitem{Coelho:2012bp}
J.~A.~Coelho, T.~Kafka, W.~Mann, J.~Schneps and O.~Altinok,
%``Constraints for non-standard interaction $\epsilon_{e \tau}V_e$ from $\nu_e$ appearance in MINOS and T2K,''
Phys. Rev. D \textbf{86} (2012), 113015
doi:10.1103/PhysRevD.86.113015
[arXiv:1209.3757 [hep-ph]].
%17 citations counted in INSPIRE as of 21 Apr 2020
 

%\cite{Miranda:2015dra}
\bibitem{Miranda:2015dra}
O.~Miranda and H.~Nunokawa,
%``Non standard neutrino interactions: current status and future prospects,''
New J. Phys. \textbf{17} (2015) no.9, 095002
doi:10.1088/1367-2630/17/9/095002
[arXiv:1505.06254 [hep-ph]].
%120 citations counted in INSPIRE as of 21 Apr 2020


%\cite{Huitu:2016bmb}
\bibitem{Huitu:2016bmb}
K.~Huitu, T.~J.~Kärkkäinen, J.~Maalampi and S.~Vihonen,
%``Constraining the nonstandard interaction parameters in long baseline neutrino experiments,''
Phys. Rev. D \textbf{93} (2016) no.5, 053016
doi:10.1103/PhysRevD.93.053016
[arXiv:1601.07730 [hep-ph]].
%31 citations counted in INSPIRE as of 21 Apr 2020

%\cite{Blennow:2015nxa}
\bibitem{Blennow:2015nxa}
M.~Blennow, S.~Choubey, T.~Ohlsson and S.~K.~Raut,
%``Exploring Source and Detector Non-Standard Neutrino Interactions at ESS$\nu$SB,''
JHEP \textbf{09} (2015), 096
doi:10.1007/JHEP09(2015)096
[arXiv:1507.02868 [hep-ph]].
%15 citations counted in INSPIRE as of 21 Apr 2020

%\cite{Masud:2016nuj}
\bibitem{Masud:2016nuj}
M.~Masud and P.~Mehta,
%``Nonstandard interactions and resolving the ordering of neutrino masses at DUNE and other long baseline experiments,''
Phys. Rev. D \textbf{94} (2016) no.5, 053007
doi:10.1103/PhysRevD.94.053007
[arXiv:1606.05662 [hep-ph]].
%42 citations counted in INSPIRE as of 21 Apr 2020


%\cite{Fukasawa:2016nwn}
\bibitem{Fukasawa:2016nwn}
S.~Fukasawa and O.~Yasuda,
%``The possibility to observe the non-standard interaction by the Hyperkamiokande atmospheric neutrino experiment,''
Nucl. Phys. B \textbf{914} (2017), 99-116
doi:10.1016/j.nuclphysb.2016.11.004
[arXiv:1608.05897 [hep-ph]].
%19 citations counted in INSPIRE as of 21 Apr 2020


%\cite{Han:2019zkz}
\bibitem{Han:2019zkz}
T.~Han, J.~Liao, H.~Liu and D.~Marfatia,
%``Nonstandard neutrino interactions at COHERENT, DUNE, T2HK and LHC,''
JHEP \textbf{11} (2019), 028
doi:10.1007/JHEP11(2019)028
[arXiv:1910.03272 [hep-ph]].
%6 citations counted in INSPIRE as of 21 Apr 2020

%\cite{Verma:2019oeb}
\bibitem{Verma:2019oeb}
S.~Verma and S.~Bhardwaj,
%``Nonstandard Interactions and Prospects for Studying Standard Parameter Degeneracies in DUNE and T2HKK,''
Adv. High Energy Phys. \textbf{2019} (2019), 8464535
doi:10.1155/2019/8464535
%2 citations counted in INSPIRE as of 21 Apr 2020

%-------------DUNE---------

  %\cite{Acciarri:2016crz}
\bibitem{Acciarri:2016crz} 
  R.~Acciarri {\it et al.} [DUNE Collaboration],
  %``Long-Baseline Neutrino Facility (LBNF) and Deep Underground Neutrino Experiment (DUNE) : Conceptual Design Report, Volume 1: The LBNF and DUNE Projects,''
  arXiv:1601.05471 [physics.ins-det].
  %%CITATION = ARXIV:1601.05471;%%
  %164 citations counted in INSPIRE as of 27 Jun 2018
  
  %\cite{Acciarri:2015uup}
\bibitem{Acciarri:2015uup} 
  R.~Acciarri {\it et al.} [DUNE Collaboration],
  %``Long-Baseline Neutrino Facility (LBNF) and Deep Underground Neutrino Experiment (DUNE) : Conceptual Design Report, Volume 2: The Physics Program for DUNE at LBNF,''
  arXiv:1512.06148 [physics.ins-det].
  %%CITATION = ARXIV:1512.06148;%%
  %581 citations counted in INSPIRE as of 29 Jan 2020

    %\cite{Abi:2020wmh}
\bibitem{Abi:2020wmh} 
  B.~Abi {\it et al.} [DUNE Collaboration],
  %``Deep Underground Neutrino Experiment (DUNE), Far Detector Technical Design Report, Volume I Introduction to DUNE,''
  arXiv:2002.02967 [physics.ins-det].
  %%CITATION = ARXIV:2002.02967;%%
  
  %\cite{Abi:2020evt}
\bibitem{Abi:2020evt} 
  B.~Abi {\it et al.} [DUNE Collaboration],
  %``Deep Underground Neutrino Experiment (DUNE), Far Detector Technical Design Report, Volume II DUNE Physics,''
  arXiv:2002.03005 [hep-ex].
  %%CITATION = ARXIV:2002.03005;%%
  %2 citations counted in INSPIRE as of 28 Feb 2020
  

% -------------NSI dune----------

%\cite{deGouvea:2015ndi}
\bibitem{deGouvea:2015ndi}
A.~de Gouvêa and K.~J.~Kelly,
%``Non-standard Neutrino Interactions at DUNE,''
Nucl. Phys. B \textbf{908} (2016), 318-335
doi:10.1016/j.nuclphysb.2016.03.013
[arXiv:1511.05562 [hep-ph]].
%90 citations counted in INSPIRE as of 21 Apr 2020


%\cite{Coloma:2015kiu}
\bibitem{Coloma:2015kiu}
P.~Coloma,
%``Non-Standard Interactions in propagation at the Deep Underground Neutrino Experiment,''
JHEP \textbf{03} (2016), 016
doi:10.1007/JHEP03(2016)016
[arXiv:1511.06357 [hep-ph]].
%90 citations counted in INSPIRE as of 21 Apr 2020


%\cite{Meloni:2018xnk}
\bibitem{Meloni:2018xnk}
D.~Meloni,
%``On the systematic uncertainties in DUNE and their role in New Physics studies,''
JHEP \textbf{08} (2018), 028
doi:10.1007/JHEP08(2018)028
[arXiv:1805.01747 [hep-ph]].
%8 citations counted in INSPIRE as of 21 Apr 2020

%\cite{Masud:2018pig}
\bibitem{Masud:2018pig}
M.~Masud, S.~Roy and P.~Mehta,
%``Correlations and degeneracies among the NSI parameters with tunable beams at DUNE,''
Phys. Rev. D \textbf{99} (2019) no.11, 115032
doi:10.1103/PhysRevD.99.115032
[arXiv:1812.10290 [hep-ph]].
%7 citations counted in INSPIRE as of 21 Apr 2020

%\cite{deGouvea:2019ozk}
\bibitem{deGouvea:2019ozk}
A.~De Gouvêa, K.~J.~Kelly, G.~Stenico and P.~Pasquini,
%``Physics with Beam Tau-Neutrino Appearance at DUNE,''
Phys.\ Rev.\ D \textbf{100} (2019) no.1, 016004
doi:10.1103/PhysRevD.100.016004
[arXiv:1904.07265 [hep-ph]].

%\cite{Bakhti:2016gic}
\bibitem{Bakhti:2016gic}
P.~Bakhti, A.~N.~Khan and W.~Wang,
%``Sensitivities to charged-current nonstandard neutrino interactions at DUNE,''
J. Phys. G \textbf{44}, no.12, 125001 (2017)
doi:10.1088/1361-6471/aa9098
[arXiv:1607.00065 [hep-ph]].
%14 citations counted in INSPIRE as of 05 Jun 2020

%\cite{Ghoshal:2019pab}
\bibitem{Ghoshal:2019pab}
A.~Ghoshal, A.~Giarnetti and D.~Meloni,
%``On the role of the $\nu_{τ}$ appearance in DUNE in constraining standard neutrino physics and beyond,''
JHEP \textbf{12} (2019), 126
doi:10.1007/JHEP12(2019)126
[arXiv:1906.06212 [hep-ph]].
%5 citations counted in INSPIRE as of 21 Apr 2020

%\cite{Blennow:2016etl}
\bibitem{Blennow:2016etl} 
  M.~Blennow, S.~Choubey, T.~Ohlsson, D.~Pramanik and S.~K.~Raut,
  %``A combined study of source, detector and matter non-standard neutrino interactions at DUNE,''
  JHEP {\bf 1608}, 090 (2016)
  doi:10.1007/JHEP08(2016)090
  [arXiv:1606.08851 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2016)090;%%
  %54 citations counted in INSPIRE as of 22 Mar 2020
  
  
  % ------- --------


  
%\cite{Blennow:2016jkn}
\bibitem{Blennow:2016jkn}
M.~Blennow, P.~Coloma, E.~Fernandez-Martinez, J.~Hernandez-Garcia and J.~Lopez-Pavon,
%``Non-Unitarity, sterile neutrinos, and Non-Standard neutrino Interactions,''
JHEP \textbf{04} (2017), 153
doi:10.1007/JHEP04(2017)153
[arXiv:1609.08637 [hep-ph]].
%98 citations counted in INSPIRE as of 21 Apr 2020  
  
  % -------ND new physics--------

%\cite{Berryman:2019dme}
\bibitem{Berryman:2019dme}
J.~M.~Berryman, A.~de Gouvea, P.~J.~Fox, B.~J.~Kayser, K.~J.~Kelly and J.~L.~Raaf,
%``Searches for Decays of New Particles in the DUNE Multi-Purpose Near Detector,''
JHEP \textbf{02} (2020), 174
doi:10.1007/JHEP02(2020)174
[arXiv:1912.07622 [hep-ph]].
%0 citations counted in INSPIRE as of 05 May 2020

%\cite{Ballett:2019bgd}
\bibitem{Ballett:2019bgd}
P.~Ballett, T.~Boschi and S.~Pascoli,
%``Heavy Neutral Leptons from low-scale seesaws at the DUNE Near Detector,''
JHEP \textbf{20}, 111 (2020)
doi:10.1007/JHEP03(2020)111
[arXiv:1905.00284 [hep-ph]].
%18 citations counted in INSPIRE as of 05 May 2020

%\cite{DeRomeri:2019kic}
\bibitem{DeRomeri:2019kic}
V.~De Romeri, K.~J.~Kelly and P.~A.~Machado,
%``DUNE-PRISM Sensitivity to Light Dark Matter,''
Phys. Rev. D \textbf{100}, no.9, 095010 (2019)
doi:10.1103/PhysRevD.100.095010
[arXiv:1903.10505 [hep-ph]].
%15 citations counted in INSPIRE as of 05 May 2020

%\cite{Ballett:2019xoj}
\bibitem{Ballett:2019xoj}
P.~Ballett, M.~Hostert, S.~Pascoli, Y.~F.~Perez-Gonzalez, Z.~Tabrizi and R.~Zukanovich Funchal,
%``$Z^\prime$s in neutrino scattering at DUNE,''
Phys. Rev. D \textbf{100}, no.5, 055012 (2019)
doi:10.1103/PhysRevD.100.055012
[arXiv:1902.08579 [hep-ph]].
%12 citations counted in INSPIRE as of 05 May 2020

%\cite{Bakhti:2018avv}
\bibitem{Bakhti:2018avv}
P.~Bakhti, Y.~Farzan and M.~Rajaee,
%``Secret interactions of neutrinos with light gauge boson at the DUNE near detector,''
Phys. Rev. D \textbf{99}, no.5, 055019 (2019)
doi:10.1103/PhysRevD.99.055019
[arXiv:1810.04441 [hep-ph]].
%13 citations counted in INSPIRE as of 05 May 2020

%\cite{Bischer:2018zcz}
\bibitem{Bischer:2018zcz}
I.~Bischer and W.~Rodejohann,
%``General Neutrino Interactions at the DUNE Near Detector,''
Phys. Rev. D \textbf{99}, no.3, 036006 (2019)
doi:10.1103/PhysRevD.99.036006
[arXiv:1810.02220 [hep-ph]].
%13 citations counted in INSPIRE as of 05 May 2020

%\cite{Ballett:2018fah}
\bibitem{Ballett:2018fah}
P.~Ballett, T.~Boschi and S.~Pascoli,
%``Searching for MeV-scale Neutrinos with the DUNE Near Detector,''
[arXiv:1803.10824 [hep-ph]].
%4 citations counted in INSPIRE as of 05 May 2020

%\cite{Miranda:2018yym}
\bibitem{Miranda:2018yym}
O.~Miranda, P.~Pasquini, M.~Tórtola and J.~Valle,
%``Exploring the Potential of Short-Baseline Physics at Fermilab,''
Phys. Rev. D \textbf{97}, no.9, 095026 (2018)
doi:10.1103/PhysRevD.97.095026
[arXiv:1802.02133 [hep-ph]].
%8 citations counted in INSPIRE as of 05 May 2020

%\cite{Choubey:2016fpi}
\bibitem{Choubey:2016fpi}
S.~Choubey and D.~Pramanik,
%``Constraints on Sterile Neutrino Oscillations using DUNE Near Detector,''
Phys. Lett. B \textbf{764}, 135-141 (2017)
doi:10.1016/j.physletb.2016.10.074
[arXiv:1604.04731 [hep-ph]].
%25 citations counted in INSPIRE as of 05 May 2020

  
%\cite{KayisTopaksu:2019dii}
\bibitem{KayisTopaksu:2019dii}
L.~Alvarez Ruso, J.~Asaadi, S.~Bolognesi, S.~Bordoni, A.~de Roeck, M.~V.~Diwan, T.~Lux, D.~Meloni, M.~Nessi, B.~Popov, E.~Radicioni, P.~Sala, F.~Sanchez and L.~H.~Whitehead,
%``Research and Development for Near Detector Systems Towards Long Term Evolution of Ultra-precise Long-baseline Neutrino Experiments,''
[arXiv:1901.04346 [physics.ins-det]].
%0 citations counted in INSPIRE as of 21 Apr 2020  

\bibitem{ND1}
Marshall, Chris. (2018, December). Near Detector Needs for Long-Baseline Physics. Zenodo. http://doi.org/10.5281/zenodo.2642327

\bibitem{ND2}
Sinclair, James. (2018, December). Liquid Argon Near Detector for DUNE. Zenodo. http://doi.org/10.5281/zenodo.2642362

\bibitem{ND3}
Mohayai, Tanaz. (2018, December). High-Pressure Gas TPC for DUNE Near Detector. Zenodo. http://doi.org/10.5281/zenodo.2642360

\bibitem{ND4}
System for on Axis Neutrino Detection
(SAND)
Status	and	Outlook, Sergio  Bertolucci, https://indi.to/Bx7Ry

\bibitem{ND5}
The DUNE Near Detector complex, Steven Manly (March 2020), https://indico.cern.ch/event/897195/contributions/3784024/attachments/2006803/3351756/DUNE\_ND\_032020.pdf


%\cite{Fogli:2002pt}
\bibitem{Fogli:2002pt}
G.~Fogli, E.~Lisi, A.~Marrone, D.~Montanino and A.~Palazzo,
%``Getting the most from the statistical analysis of solar neutrino oscillations,''
Phys. Rev. D \textbf{66} (2002), 053010
doi:10.1103/PhysRevD.66.053010
[arXiv:hep-ph/0206162 [hep-ph]].
%348 citations counted in INSPIRE as of 12 May 2020

     %\cite{Huber:2004ka}
\bibitem{Huber:2004ka} 
  P.~Huber, M.~Lindner and W.~Winter,
  %``Simulation of long-baseline neutrino oscillation experiments with GLoBES (General Long Baseline Experiment Simulator),''
  Comput.\ Phys.\ Commun.\  {\bf 167}, 195 (2005)
  doi:10.1016/j.cpc.2005.01.003
  [hep-ph/0407333].
  %%CITATION = doi:10.1016/j.cpc.2005.01.003;%%
  %518 citations counted in INSPIRE as of 08 Jul 2019
  
  %\cite{Huber:2007ji}
\bibitem{Huber:2007ji}
  P.~Huber, J.~Kopp, M.~Lindner, M.~Rolinec and W.~Winter,
  %``New features in the simulation of neutrino oscillation experiments with GLoBES 3.0: General Long Baseline Experiment Simulator,''
  Comput.\ Phys.\ Commun.\  {\bf 177} (2007) 432
  doi:10.1016/j.cpc.2007.05.004
  [hep-ph/0701187].
  %%CITATION = doi:10.1016/j.cpc.2007.05.004;%%
  %431 citations counted in INSPIRE as of 01 Jun 2019
  
   %\cite{Kopp:2006wp}
\bibitem{Kopp:2006wp} 
  J.~Kopp,
  %``Efficient numerical diagonalization of hermitian 3 x 3 matrices,''
  Int.\ J.\ Mod.\ Phys.\ C {\bf 19}, 523 (2008)
  doi:10.1142/S0129183108012303
  [physics/0610206].
  %%CITATION = doi:10.1142/S0129183108012303;%%
  %76 citations counted in INSPIRE as of 22 Mar 2020 
  

  
\bibitem{fluxes}
“http://home.fnal.gov/ljf26/DUNEFluxes/”

    %\cite{Alion:2016uaj}
\bibitem{Alion:2016uaj} 
  T.~Alion {\it et al.} [DUNE Collaboration],
  %``Experiment Simulation Configurations Used in DUNE CDR,''
  arXiv:1606.09550 [physics.ins-det].
  %%CITATION = ARXIV:1606.09550;%%
  %54 citations counted in INSPIRE as of 08 Jul 2019


  

  
  
  
  \end{thebibliography}
